Direct limits for scalar field dark matter from a gravitational-wave detector

The nature of dark matter remains unknown to date; several candidate particles are being considered in a dynamically changing research landscape. Scalar field dark matter is a prominent option that is being explored with precision instruments, such as atomic clocks and optical cavities. Here we report on the first direct search for scalar field dark matter utilising a gravitational-wave detector, which operates beyond the quantum shot-noise limit. We set new upper limits for the coupling constants of scalar field dark matter as a function of its mass, by excluding the presence of signals that would be produced through the direct coupling of this dark matter to the beamsplitter of the GEO$\,$600 interferometer. The new constraints improve upon bounds from previous direct searches by more than six orders of magnitude, and are in some cases more stringent than limits obtained in tests of the equivalence principle by up to four orders of magnitude. Our work demonstrates that scalar field dark matter can be probed or constrained with direct searches using gravitational-wave detectors, and highlights the potential of quantum-enhanced interferometry for dark matter detection.

==> sections/alternatives.tex <==
\section{Rewrite}
\subsection{Spectral estimation (Section 3A)}
NOTE: This is just a different presentation of mostly Sander's writing for section 3A. Please feel free to ignore/cherry-pick it at will.

In order to tune our spectral estimation  to the resolution of the DM signal, we applied a modified version of the LPSD algorithm outlined in \cite{trobs_improved_2006}. This algorithm is designed to perform a power spectral density (PSD) calculation with a logarithmic bin spacing in the frequency domain. To perform our analysis we modified the LPSD algorithm to enforce a bandwidth of $r_j = f_j \times 10^{-6}$ for the entire frequency domain, regardless of number of desired averaged segments. This required time series of length $>20,000$ seconds.

We acquired seven continuous sections of strain data from the GEO600 detector \cite{Dooley_2016}. These time series were recorded at quarterly intervals during the observing runs in 2016 and 2019. The data was recorded at a sample rate of $16384 Hz$ and each time series was on the order of $10^5$ seconds in length.

We performed this analysis for $5098893$ frequency bins spaced logarithmically between $50$ and $8192 Hz$. The LPSD process is then as follows, for each frequency bin:

\begin{itemize}
  \item The time series is divided into $N_f$ overlapping segments $S_f^k(t)$ with a length equal to the expected coherence time $\tau_\text{coh}(f)$ of the signal at a frequency $f$ (where $N_f=\lfloor \frac{T-\tau_\text{coh}(f)}{\tau_\text{coh}(f) (1-\xi)} \rfloor$, $\xi\in[0,1]$ is the fractional overlap of the segments, and $k\in [1, N_f]$). For our analysis we used an overlap of $\xi = 0.2$
  \item Each segment is then windowed with a Kaiser window, $\beta = 30$
  \item For each windowed segment a Discrete Fourier Transform (DFT) is calculated:
  \begin{equation}
      a^k(f) = \sum_{t=0}^{T_\mathrm{DFT}} W_f(t)\, S_f^k(t)\, \mathrm{e}^{2\pi i f t},  
  \end{equation}
        where $T_\mathrm{DFT}=\tau_\text{coh}(f)$, where $a^k(f)$ is then the complex spectral estimate at frequency $f$ for the $k^\text{th}$ segment.
  \item The complex spectral estimate is then averaged over all segments and normalised to return the power spectrum at frequency f:
  \begin{equation}
      P(f)=\frac{C}{N_f}\sum_{k=1}^{N_f}|a^k(f)|^2,
  \end{equation}
       where $C$ is the normalisation factor.
  \item The square root is then taken to provide the desired amplitude spectrum:
  \begin{equation}
      A(f)= \sqrt{P(f)}
  \end{equation}
\end{itemize}

As each frequency bin can be calculated independently, the process allows for high levels of parallelisation. The calculation speed for each frequency bin varies with respect to the length of the segment, longer for lower frequencies. The calculation time for a time series of length T ~ 70,000 seconds is approximately 800 days on a single Intel Xenon Processor: E5-2680 v3 @ 2.50GHz.


==> sections/scratch.tex <==
OPL difference:

\begin{align}
    \delta(L_x - L_y) &= \frac{1}{\cos(\theta_r')}(l+\delta l)(n+\delta n) - \frac{1}{\cos(\theta_r)}ln \\
    &+\frac{\sin(45^\circ-\theta_r')}{\cos(\theta_r')}(l+\delta l) - \frac{\sin(45^\circ-\theta_r)}{\cos(\theta_r)}(l) \\
    & -\sqrt{2}\delta l (\frac{1}{2} + \tan(45^\circ - \theta_r'))
\end{align}

OPL difference for $\theta_r=\theta_r'=45^\circ$

\begin{equation}
     \delta(L_x - L_y) \approx \sqrt{2}(l\delta n + n\delta l + \delta l \delta n - \delta l/2)
\end{equation}

==> sections/sec_Method_Validation.tex <==
\section{Validation of Methods}\label{sec:methodval}
To validate several aspects of our analysis methods, we simulated dark matter (DM) signals and injected them into several sets of GEO\,600 data. The DM signals were created by superposing $\sim10^2$ sinusoids at frequencies linearly spaced around a centre frequency (the simulated Doppler-shifted DM Compton frequency), where the amplitude of each sinusoid is given by the quasi-Maxwellian DM line shape proposed in \cite{derevianko_detecting_2018} scaled by a simulated DM coupling constant; the relative phases of the sinusoids are randomised to capture the thermalisation of the scalar field DM.

To test the spectral estimation, signal search, and candidate rejection, an injection of simulated DM signals into several data sets was performed, where the frequency, amplitude, and number of signals was masked to the authors. All injected signals were recovered at their Compton frequency and at an amplitude corresponding to the hypothetical coupling constant, and were subsequently identified through cross-checks between spectra as persistent candidate DM signals.


\begin{figure}
    \includegraphics[width=0.45\textwidth]{figures/Ampl_Scaling.eps}
    \caption{caption EDIT}
    \label{fig:ampl_scaling}
\end{figure}
[Here we will discuss an additional investigation into the scaling of the recovered amplitude and SNR of simulated DM signals with the frequency bin width, which shows that the maximal SNR is obtained when the bin width $\approx$ DM linewidth as proposed. This analysis also validates the rejection of the one remaining candidate peak (see above) based on its scaling with DFT length.]

% \phil{Here is my draft. Please feel free to desecrate it at will}
% \subsection{Blind Signal Injection} \label{Blind injection}
% To check our peak elimination process we created spectra containing simulated Dark Matter signals. These signals were produced by randomly selecting a frequency and amplitude, then creating a range of sine waves following the amplitude distribution outlined in \cite{derevianko_detecting_2018}. The peaks of the signals were Doppler shifted to account for XXX \phil{I can't remember if it's Earths motion wrt Sun or Galactic center? Is there a good source to quote for the actual shift here?}. Two spectra were created six months apart to allow for the maximum Doppler shift. The signals were then summed with the original data.

% The LPSD algorithm was then applied to the data and a catalogue of persistent peaks was drawn up as outlined in section \ref{method-signalsearch}. This process was performed blind with no knowledge of the number of signals, or the characteristics of those signals. At the end of this process there were 7209 candidate signals. Upon opening the box we found that there had been five injected signals. All five signals were found in the candidate catalogue to within one bin width of the injected signal frequency. The recovered signal amplitudes matched those of the injection. \phil{These matched to max difference of 3\%. I assume that's enough to make this statement, if we want it}

% \subsection{Noise Floor Scaling} \label{Floor scaling}
% To test the significance of the recovery amplitude we created Gaussian noise and calculated LPSD spectra from them at different resolutions. We compared the DFT period from the LPSD to the recovered amplitude and standard deviation. We found that the recovered amplitude of the noise is inversely proportional to the square root of the period of the DFT. The same is true for the recovered standard deviation. The constants of proportionality are X \& Y. \phil{We are still trying to outline these} \phil{It might be be better to give them as an equation though}

% We performed the same analysis with time series with injected signals. Two spectra, one with a DM curve injected with amplitude distribution as in \cite{derevianko_detecting_2018} and another with a single sine wave injected. These were then recovered at different resolutions in order to check how the significance of the recovered peak varies with the LPSD resolution. \phil{I'll add a plot of this once it's done}

% \phil{Do we want to include this just for Gaussian noise or GEO noise too? If you do want this then please chop and choose from the previous paragraph as needed.}

%[Here we could show the scaling of peak height w.r.t. noise height (SNR) as function of DFT length. We can also show recovery and detection/persistence of simulated peaks in spectra]

% % Phil's ideas:

% To test the validity of the search, simulated DM signals were injected into the data. These signals followed the distribution defined in equation XXX from \cite{derevianko_detecting_2018}. These signals were injected with randomly selected frequency and amplitude. The signals were then injected into different time series. The frequency of the DM curve was modulated in each data segment to account for the Doppler shift from the Earth's position relative to the galactic center. Each modified time series was then run through the LPSD again. The process was done double-blind with no knowledge of the number of signals injected or the characteristics of the signals.

% List of possibilities from here:
% \begin{itemize}
%     \item Layout blind injection recovery \& findings
%     \item Missed found plot for 100 injected signals? This would take about a week to run. We could inject the signals at lower resolution (i.e. the curve split into 100, not 500 bins on injection). We could reduce the section of frequency space and run a full LPSD on it. Then we recover from the injection at different sensitivities. I would need to spend some time calculating limits for injected amplitudes first
%     \item Plot for the DM curve vs sine wave recovered at different resolutions. See: \url{https://ligo.gravity.cf.ac.uk/~philip.relton/projects/geo-dark-matter/science_runs/monochrome_injection/test_10-5/Recovered_peak_significance.png}
%     \item Plot from the same DM vs sine study, but showing the shape of the curve at different resolutions. Something like this: \url{https://ligo.gravity.cf.ac.uk/~philip.relton/projects/geo-dark-matter/science_runs/monochrome_injection/test_10-5/all_resolutions/DM_10-5_injected_closest.png}
%     \item Plot showing the curve recovered at $>10^{-6}$ with two time series 6 months apart recovered. This would show the curve shape and the Doppler shift
% \end{itemize}

==> sections/sec_Methods.tex <==
\section{Methods}\label{sec:methods}
\begin{figure*}[ht]
\centering
\includegraphics[scale=0.35]{figures/Paper_95_bmed_Peaks_50-5800Hz_03-03-2021_1415.eps}
\caption{A typical amplitude spectrum (black) produced with frequency bins that are tuned to the expected dark matter linewidth using the modified LPSD technique. The noise spectrum was estimated at each frequency bin from neighbouring bins to yield the local noise median (blue) and 95\% confidence level (green). Peaks (red) above this confidence level were considered candidates for DM signals and subjected to follow-up analysis.}
\label{fig:peak_selection}
\end{figure*}

%\subsection{Spectral estimation}
We performed spectral analysis on seven $T\sim 10^5$~s segments of strain data from the GEO\,600 interferometer~\cite{Dooley_2016} (acquired in 2016 and 2019) using a modified version of the LPSD technique ~\cite{trobs_improved_2006, trobs2009improved}, which was designed to produce spectra with logarithmically spaced frequencies. Using this algorithm to perform discrete Fourier transforms (DFT) with a frequency dependent length, we created spectra in which each frequency bin was made to have a width equal to the Doppler-broadened linewidth of potential DM signals. This method yields in theory the maximum attainable signal-to-noise ratio (SNR) given a certain amount of data (see Sec.~\ref{sec:nature_meth})~\cite{miller_adapting_2020,derevianko_detecting_2018}. A matched filtering approach is not feasible as the phase of the signal varies stochastically.

%\subsection{Candidate signal search} \label{method-signalsearch}
We analysed the amplitude spectra of all seven strain data segments %of length $T\sim 10^5$~s 
for the presence of DM signals by looking for significant peaks in the underlying noise. Peaks were considered candidates when there was a less than $1\%$ probability of the local maximum being due to noise, where we compensated for the look-elsewhere effect using a large trial factor ($\sim10^{6}$). 
% To determine this probability for every peak, the noise was assumed to be Gaussian with a frequency-dependent expectation value and variance. The local noise parameters were estimated at every frequency bin from $w=5\cdot10^4$ neighbouring bins. This method allows the underlying noise distribution to be estimated in a way that is independent of narrow ($\ll w$) spectral features (such as those due to mechanical excitation of the mirror suspensions), under the assumption that the underlying noise spectrum is locally flat (that is, the auto-correlation length of the noise spectrum is assumed to be $\gg w$)\cite{Note_on_w}.

This analysis found %$\approx 3.5\pm 0.5\cdot 10^4$ 
$\sim 10^4$ peaks above the 95\% confidence level ($\gtrsim 5.6 \sigma$), where the total error includes a frequency dependent amplitude calibration error of up to $30\%$ inherent to GEO\,600 data \cite{GEOcal_2019}. The frequency and amplitude stability of the peaks in time was then evaluated by cross-checking all candidates between spectra. Candidate peaks were rejected if their centre frequencies differed between spectra by more than the Doppler shift expected from the Earth's motion around the Sun \cite{freese_annual_2013}. Peaks were also rejected if their amplitude changed significantly ($\gtrsim 5 \sigma$) between spectra. 
%between spectra by more than an amount expected due to the underlying noise. Specifically, peaks that changed amplitude between spectra were only eliminated when there was a less than $1\%$ ($\gtrsim 5 \sigma$) probability that the amplitude change was due to noise (compensated for the look-elsewhere effect).%, so that on average only one peak would be falsely rejected if all cross-checks are performed 100 times). 

Using this procedure, we eliminated all but 14 candidate peaks, where the vast majority ($>99\%$) of peaks were rejected because they did not appear in all data sets within the centre frequency tolerance.

%\subsection{Follow-up analysis of candidates}
These 14 candidate peaks were subjected to further analysis to investigate if their properties matched that of a DM signal. 13 of the peaks were found to have insufficient width to be caused by DM ($\Delta f_\mathrm{peak}/\Delta f_\mathrm{DM}\lesssim 10$, see Sec.~\ref{sec:nature_meth}). %\vivien{This is a good argument, but it has a significant impact on the results. So I think it'd be best to give number, what's the width of those peaks (average, maximum) compared to the smallest width one can expect from DM, to help the reader get behind this argument}.
% Investigation of each of these candidates found that shifting the bin centre frequencies by an amount much smaller than the expected linewidth of DM signals of that frequency and amplitude and recomputing the spectra did not reproduce the peak \cite{Note_on_peaks}. Specifically, the ratio of observed and expected peak width was $\Delta f_\mathrm{peak}/\Delta f_\mathrm{DM}\lesssim 10$ for these 13 peaks. %\footnote{Additional work revealed these 20 candidate peaks were not present in spectra created using the same data and the same LPSD algorithm implemented in a different programming language, whereas the noise floor and other spectral features were reproduced identically. These peaks are therefore likely artefacts of the numerical implementation of the LPSD technique.}.
The remaining candidate peak was also ultimately rejected, as although it appeared to have sufficient frequency spread to be a DM signal, additional analysis showed this signal has a coherence time much greater than that expected for a DM signal of that frequency ($\tau_c^\mathrm{peak}/\tau_c^\mathrm{DM}>10$, see Sec.~\ref{sec:nature_meth}).
% ; i.e. the height of the peak did not decrease for DFT lengths more than an order of magnitude greater than the expected DM coherence time.



==> sections/sec_Results.tex <==
\section{Results}\label{sec:results}
\begin{figure*}[!htb]
  \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/Paper_phot_square_Lambda_Excl._50-5800Hz_m_phi=1e-20-1e-05eV.eps}
    %\caption{Constraints on the parameters of scalar field DM interacting linearly with}
    \label{fig:constraints_phot}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/Paper_elec_square_Lambda_Excl._50-5800Hz_m_phi=1e-20-1e-05eV.eps}
    %\caption{wewefsdf}
      \label{fig:constraints_el}
  \end{minipage}
  \caption{Constraints on the coupling parameters $\Lambda_\gamma$, $\Lambda_e$ of scalar field DM interacting linearly with respectively the electromagnetic (left) and electron field (right) as a function of the field's mass $m_\phi$. The green regions denote the parameter space excluded at a 95\% confidence level in the current study through the spectral analysis of data from the GEO\,600 GW detector. The thin red regions show existing constraints of scalar field DM obtained with the resonant-mass AURIGA detector \cite{branca_search_2017}. The other coloured regions represent previous constraint from other direct searches \cite{savalle_searching_2021,aharony_constraining_2019,van_tilburg_search_2015,hees_searching_2016}. The grey regions correspond to previous constraints on general fifth-forces from tests of the equivalence principle \cite{leefer_search_2016} in earth-based (Rot-Wash) \cite{smith_short-range_1999} and space-based (MICROSCOPE) \cite{berge_microscope_2018}  experiments.}
  \label{fig:constraints}
\end{figure*}

Having determined that all significant peaks in the amplitude spectrum %that are above the noise at a confidence level of $>99\%$
are not caused by scalar field DM, we set constraints on the parameters of such dark matter at a 95\% confidence level (corresponding to $5.6\sigma$ above the noise floor), using Eq.~\ref{eq:full_signal}. The results for the photon and electron coupling parameters as a function of field mass are given in Fig.~\ref{fig:constraints}.
% These constraints cover the mass range between $\approx {2\cdot10^{-13}\;\mbox{--}\;2\cdot10^{-11}}$~eV, and improve over the current upper limits on both $\Lambda_e$ and $\Lambda_\gamma$ set through atomic spectroscopy experiments \cite{aharony_constraining_2019,stadnik_can_2015,stadnik_enhanced_2016} by more than six orders of magnitude. In addition,  our results constrain the scalar DM-electron coupling constant $\Lambda_e$ at a level one order of magnitude lower than previous bounds from tests of the equivalence principle \cite{smith_short-range_1999,hees_violation_2018}. 

These results assume a local dark matter density $\rho_\mathrm{CDM}=0.3$~GeV/cm$^3$. This is a conservative estimate; slightly higher values ($\rho_\mathrm{CDM}\approx 0.4$~GeV/cm$^3$) are reported in literature for the standard smooth DM halo model \cite{freese_annual_2013}. Models in which DM forms a relaxion halo \cite{graham_cosmological_2015,kolb_axion_1993} predict local DM overdensities of up to $\rho_\mathrm{RH}/\rho_\mathrm{CDM}\leq 10^{16}$ \cite{savalle_novel_2019}. Our results impose significantly more stringent constraints on the coupling constants for higher assumed values of the DM density $\rho_\mathrm{A}>\rho_\mathrm{CDM}$: the constraint becomes more stringent by a factor $(\rho_\mathrm{A}/\rho_\mathrm{CDM})^{1/2}$ (see Eq.~\ref{eq:full_signal}). 
